Lyapunov stabilization for nonlocal traffic flow models

Using a nonlocal second-order traffic flow model we present an approach to control the dynamics towards a steady state. The system is controlled by the leading vehicle driving at a prescribed velocity and also determines the steady state. Thereby, we consider both, the microscopic and macroscopic scales. We show that the fixed point of the microscopic traffic flow model is asymptotically stable for any kernel function. Then, we present Lyapunov functions for both, the microscopic and macroscopic scale, and compute the explicit rates at which the vehicles influenced by the nonlocal term tend towards the stationary solution. We obtain the stabilization effect for a constant kernel function and arbitrary initial data or concave kernels and monotone initial data. Numerical examples demonstrate the theoretical results.

==> macros.tex <==
\usepackage[english]{babel}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{a4wide}
\usepackage{verbatim}
\RequirePackage{ifthen}
\RequirePackage[T1]{fontenc}
\RequirePackage{color}
\RequirePackage{listings} 
\RequirePackage{epstopdf}
\RequirePackage{emptypage}
\RequirePackage[nolist]{acronym}
\RequirePackage{multirow}
\RequirePackage{enumerate,enumitem}
\RequirePackage{caption}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta}
\RequirePackage{latexsym,amscd,makeidx}
\RequirePackage{exscale}
\RequirePackage{mathrsfs}
\RequirePackage{hyperref}
\RequirePackage{url}
\RequirePackage{booktabs}
\RequirePackage{esdiff}
\RequirePackage{listings}
\RequirePackage{tabularx}
\RequirePackage[numbers]{natbib}
\RequirePackage{verbatim}
\RequirePackage{comment}
%\RequirePackage{cite}
\RequirePackage{cleveref}
\crefname{equation}{}{}
\Crefname{Equation}{}{}
\usepackage{pgfplots} 
\usepackage{pgfgantt}
\usepackage{pdflscape}
%\usepackage[notref,notcite]{showkeys}
\pgfplotsset{compat=newest} 
\pgfplotsset{plot coordinates/math parser=false}
\numberwithin{equation}{section}
% Switch: Hide or show comments
	\newif\ifshowcomments								
%	\showcommentstrue				% show comments
	\showcommentsfalse				% hide comments


% Definition of environments
	\definecolor{mygrey}{gray}{0.65}
	
	% Detailed comments
	\ifshowcomments
		% Display comments in a specified environment
		\newenvironment{bcomment}[1][]
	 	{~\\~\\ \begin{color}{mygrey}\begin{small}\noindent\textbf{COMMENT: #1}~\\}
	 	{\end{small}\end{color}~\\~\\}
	\else
		% Hide comments
	 	\excludecomment{bcomment}
	\fi
	% Inline-Comments
	
	\ifshowcomments
		\newcommand{\scomment}[1]{{\color{mygrey} [#1]}}  % small comments within lines
	\else
		\newcommand{\scomment}[1]{\iffalse #1 \fi}
	\fi

% Adjust sign of a number for the tikz picture of the grid 
	\newcommand\checkindex[1]{
		\pgfmathsetmacro{\var}{#1}
		\pgfmathparse{ifthenelse(\var==0, "",ifthenelse(\var>0, "+#1","#1"))} \pgfmathresult}%

%For tikz plots
\newlength\fwidth

% Create 'todo' marker (called by \todo{TEXT})
\newcommand{\margtodo}
{\marginpar{\textbf{\textcolor{red}{ToDo}}}{}}
\newcommand{\todo}[1]
{{\textbf{\textcolor{red}{-- \margtodo{}#1 --}}}{}}

\newcommand{\margidea}
{\marginpar{\textbf{\textcolor{orange}{Idea}}}{}}
\newcommand{\idea}[1]
{{\textbf{\textcolor{orange}{-- \margidea{}#1 --}}}{}}

\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\BV}{BV}

\RequirePackage{amsthm}
\theoremstyle{plain}						% Default
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{remark}[theorem]{Remark}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

%%%Notation:
%Define some shortcuts
%% math calligraphy
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
%% math blackboard bold
%\newcommand{\A}{\mathbb{A}}
%\newcommand{\B}{\mathbb{B}}
%\newcommand{\C}{\mathbb{C}}
%\newcommand{\D}{\mathbb{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
%\newcommand{\I}{\mathbb{I}}
%\newcommand{\J}{\mathbb{J}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\N}{\mathbb{N}}
%\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
%\newcommand{\T}{\mathbb{T}}
%\newcommand{\U}{\mathbb{U}}
%\newcommand{\V}{\mathbb{V}}
%\newcommand{\W}{\mathbb{W}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\Y}{\mathbb{Y}}
\newcommand{\Z}{\mathbb{Z}}

%% New commands
\newcommand{\OAP}{$(\Omega,\mathcal{A},P)$}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\Ind}{\mathds{1}}
\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
\newcommand{\sign}{\operatorname{sgn}}
\newcommand{\Div}{\operatorname{div}}
\newcommand{\lano}{\mathrm{o}}
\newcommand{\lanO}{\mathrm{O}}
\newcommand{\dint}{\displaystyle\int}
\newcommand{\dsup}{\displaystyle\sup}
\newcommand{\dsum}{\displaystyle\sum}
%\newcommand{\BV}{\operatorname{BV}}
\newcommand{\TV}{\operatorname{TV}}
%System
\newcommand{\consys}{\cQ}

%Indicies
\newcommand\half{{\frac12}}
\newcommand\jmo{{j-1}}
\newcommand\jmh{{j-\half}}
\newcommand\jpmh{{j\pm\half}}
\newcommand\jph{{j+\half}}
\newcommand\jpo{{j+1}}
\newcommand{\jpk}{{j+k}}
\newcommand{\jpko}{{j+k+1}}
\newcommand{\kmo}{{k-1}}
\newcommand\npo{{n+1}}

%Step sizes
\newcommand{\Dx}{\Delta x}
\newcommand{\Dt}{\Delta t}

%Computations
\newcommand\dx{\mathit{dx}}
\newcommand\dy{\mathit{dy}}
\newcommand\dt{\mathit{dt}}
\newcommand\ds{\mathit{ds}}
\newcommand{\norm}[1]{{\left\|#1\right\|}}
\newcommand{\abs}[1]{{\left|#1\right|}}

%Spaces:
\newcommand{\LinfR}{{L^\infty(\R)}}
\newcommand{\LinfRR}{{L^\infty(\R;\R)}}
\newcommand{\LoneR}{{L^1(\R)}}
\newcommand{\LoneRR}{{L^1(\R;\R)}}
\renewcommand{\L}[1]{L^{#1}}
\newcommand{\Lloc}[1]{L^{#1}_{loc}}

%Nonlocal look ahead distance for the source term
\newcommand{\nds}{{\nu}}
%Kernel Function for source term
\newcommand{\ws}{W_{\nds}}
%Nonlocal look ahead distance for the transport term
\newcommand{\ndt}{{\eta}}
%Kernel Function for transport term
\newcommand{\wt}{W_{\ndt}}
\newcommand{\twt}{\mathcal{W}_{\ndt}}
%Upperbound for discrete convolution
\newcommand{\Ne}{N_\ndt}

%Kernel Functions transport:
\newcommand{\wtcon}{\wt^{\text{const.}}}
\newcommand{\wtlin}{\wt^{\text{lin.}}}
\newcommand{\wtconcave}{\wt^{\text{conc.}}}
%Coupling function:
\newcommand{\coupling}{g}
\newcommand{\newg}{\Gamma}
%Test functions
\newcommand{\testf}{\phi}

%Discrete rho
\newcommand{\dr}{\rho^{\Dx}}
%N_T Time iterations scheme
\newcommand{\NT}{{N_T}}

%n for different \Dx values for convergence
\newcommand{\nconv}{\mathcal{N}}

%Characteristics
\newcommand{\chr}{X}
%Characteristics of rho, t0, x0
\newcommand{\chrptxz}{{\chr_\rho[t_0,x_0]}}


%Paper Maximum Principle
\renewcommand{\P}{P}
\newcommand{\w}{w}
\newcommand{\coeff}{\mu}
\newcommand\opt{{\text{opt}}}
\newcommand\brho{{\bar\rho}}
\renewcommand{\S}{SI}

% quadrature
\newcommand{\qn}{{\nu}}
\newcommand{\nqn}{{J}}
\newcommand{\qw}{{h}}
\newcommand{\qwn}{\qw_\qn}
\newcommand{\qvar}{{y}}

%Order of reconstruction
\newcommand{\g}{o}
\newcommand{\GPopt}{O}


%For networks
\newcommand{\road}{E}
\newcommand{\roadind}{e}
\newcommand{\vertice}{Z}
\newcommand{\verticeind}{z}
\newcommand{\Ro}{\rho^{\max}_1}
\newcommand{\Rt}{\rho^{\max}_2}
\newcommand{\Rtr}{\rho^{\max}_3}
\newcommand{\Rr}{\rho^{\max}_\roadind}
\newcommand{\po}{\rho_1}
\newcommand{\pt}{\rho_2}
\newcommand{\pe}{\rho_\roadind}
\newcommand{\roadbeginohne}{a}
\newcommand{\roadbegin}{\roadbeginohne_\roadind}
\newcommand{\roadendohne}{b}
\newcommand{\roadend}{\roadendohne_\roadind}
\newcommand{\incoming}{\mathcal{I}}
\newcommand{\incomingind}{i}
\newcommand{\NI}{N_\incoming}
\newcommand{\outgoing}{\mathcal{O}}
\newcommand{\outgoingind}{o}
\newcommand{\NO}{N_\outgoing}
\newcommand{\distMatrix}{\mathbb{A}}
\newcommand{\distpar}{\alpha}
\newcommand{\priopar}{q}
\newcommand{\lipschitzcoupling}{{L_\coupling}}
\newcommand{\totaltraveltime}{TTT}
\newcommand{\outflow}{O}
\newcommand{\congestionmeasure}{CM}


\newcommand{\newgo}{\newg_{\outgoingind}}

%Multilane
\newcommand{\borho}{\boldsymbol{\rho}}
\newcommand{\bodr}{\boldsymbol{\rho}^{\Dx}}
\newcommand{\drl}{\rho^{\Dx,\ell}}
\newcommand{\caratt}[1]{{\chi_{\strut#1}}}
\newcommand{\spt}{\mathop{\rm supp}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\boV}{\boldsymbol{V^\nds}}
%Characteristics of bold rho and \ell
\newcommand{\chrl}{\chr_{\borho,\ell}}
\newcommand{\chrb}{\chr_{\borho}}

%GARZ
%Lagrangian marker
\newcommand{\lm}{\omega}
\newcommand{\vg}{u}
\newcommand{\VG}{U}

\newcommand{\jan}[1]{\textcolor{orange}{[Jan: #1]}}
